How Powerful are Interest Diffusion on Purchasing Prediction: A Case Study of Taocode

A taocode is a kind of specially coded text-link on Taobao(the world's biggest online shopping website), through which users can share messages about products with each other. Analyzing taocodes can potentially facilitate understanding of the social relationships between users and, more excitingly, their online purchasing behaviors under the influence of taocode diffusion. This paper innovatively investigates the problem of online purchasing predictions from an information diffusion perspective, with taocode as a case study. Specifically, we conduct profound observational studies on a large-scale real-world dataset from Taobao, containing over 100M Taocode sharing records. Inspired by our observations, we propose InfNet, a dynamic GNN-based framework that models the information diffusion across Taocode. We then apply InfNet to item purchasing predictions. Extensive experiments on real-world datasets validate the effectiveness of InfNet compared with 8 state-of-the-art baselines.

==> model_old.tex <==
\section{Model: \textit{\modelname~}}
\label{sec:model}

\begin{figure*}[ht]
	\centering
	\includegraphics[width=1.0\textwidth]{./fig/test.pdf}
	\caption{Overview of \modelname.
		\small
		\czq{fix model figure and caption@xuanwen}
		\normalsize
	}
	\label{fig:model:overview}
\end{figure*}

\begin{table}[t!]
	\caption{Notation table.
		\small Note that all those notations can be incorporated with a super- or subscript $t$
		which indicates the time step.
		\normalsize
	}
	\begin{tabular}{c|p{0.75\columnwidth}}  
		\toprule
		Notation & Description\\
		\hline
		$\mathcal{G}$& the interest diffusion network\\ \hline
		$\mathcal{G}^q$& the sub-network of $\mathcal{G}$ for a query $q$ \\ \hline
		$\mathbf{X},x_u$& node representations in the node-aware \modelname~(\modelname-N), where $u$ denotes a specific user\\\hline
		$\mathbf{H},h_u$& node representations in the edge-aware \modelname~(\modelname-E), where $u$ denotes a specific user\\\hline
		$E,e_{uv}$& edge representation in \modelname-E, where $e_{uv}$ denotes a specific directed edge between user $u$ and $v$\\\hline
		$\mathcal{E}_{in}, \mathcal{E}_{out}$& the set of in/out edges of the interest diffusion (sub-) network\\\hline
		$\mathcal{E}^{u}_{in}, \mathcal{E}^{u}_{out}$& the set of in/out edges of a user $u$ in the interest diffusion (sub-) network\\\hline
		$\mathcal{S}_u$& the set of \textit{sender nodes} that share \tcode~to $u$ in the network, i.e., neighbors of in edges.\\\hline
		$\mathcal{R}_u$ & the set of \textit{receiver nodes} that receive \tcode~from $u$ in the network, i.e., neighbors of out edges\\\hline
		$\mathcal{N}_u$& all neighbors of node $u$ in the diffusion network\\\hline
		$a_{uv}$& attention weight of edge $e_{uv}$\\
		\bottomrule
	\end{tabular}
	\label{tbl:notations}
\end{table}

In this section, we introduce the proposed model, Bi-directional Graph Attention Networks (\modelname), 
for modeling structural and temporal dynamics of \tcode~ diffusions in the interest diffusion networks. 
Given the input of a purchasing query at a specific time step that contains the targeting user and item,
our framework first builds a sequence of dynamic sub-networks for each query,
where the features of nodes and edges are carefully extracted from the targeting user and item;
then we apply the \textit{edge-aware GNN} to aggregate the dynamic edge attributes across the time into node features,
and use \textit{node-aware bi-directional GAT} to capture the structural characteristics by aggregating neighbors' information.
Finally, the graph-level representations along with features of the targeting item are feed into the outer classifier,
to predict whether the target user will make a purchase on the item during the given time span. 
The framework overview is illustrated in \figref{fig:model:overview},
and to make it clear, we summarize the notations of our model in \tableref{tbl:notations}.
%Motivated by Section 3, 

\subsection{Preprocessing: sub-graph construction}
\label{subsec:sub-graph}
For each purchasing query $q=(u, p, t)$ and the whole dynamic interest diffusion network $\mathcal{G} = \{\mathcal{G}_1, \cdots, \mathcal{G}_t\}$,
we first build a sequence of sub-graphs $\mathcal{G}^q$ of $\mathcal{G}$ to conduct the end-to-end graph classification, i.e., purchasing prediction of query $q$.
The process of constructing the sub-networks can be described as follows:
\begin{itemize}[leftmargin=*]
	\item \vpara{seed node sampling:} we define the target user $u$ and its neighbors $\mathcal{S}_u(p)$ as the set of seed nodes,
	denoted as $\{u\} \bigcup \mathcal{S}_u(p)$, Where $\mathcal{S}_u(p)$ is the set of \textit{sender nodes} that shares item $p$ to $u$.
	\item \vpara{sub-network construction:} given the set of seed nodes, we adopt a breath-first search (BFS) strategy to sample the nodes in  $\mathcal{G}_t^q$
	from each original diffusion network $\mathcal{G}_t$, by searching for two-hop neighbors, i.e., search breadth is set as two;
	and there exists an edge for two nodes $(u, v)$ in $\mathcal{G}_t^q$ if the user $u$ shares some product $p$ to $v$ at the time step $t$.
	Node and edge features would be defined the same as in $\mathcal{G}_t$.
\end{itemize}
And algorithm formulations can be referred in \algref{alg:sub-graph sample}.

Based on the graph structures, there are sufficient node and edge attributes.
The node features of a user $u$, denoting as $Attr(u)$, has two parts. 
The first part is the user's purchasing histories which are independent with the diffusion networks, 
i.e., the price she pays for products in the past year;
and the other part is a one-hot vector, indicating whether this node is the target user in the query or it is among the seed nodes,
which can help our model better identify the nodes that need to be focused~\cite{zhang2018link}. 

\begin{algorithm}[t!]
	\caption{Diffusion sub-graph construction}
	\label{alg:sub-graph sample}
	\begin{algorithmic}[1]
		\REQUIRE purchasing query $q=(u,p,t)$, \\original interest diffusion network $\mathcal{G}_t$\\
		\ENSURE  diffusion sub-network $\mathcal{G}_t^q$ of query $q$\\
		\STATE Initialize the set of seed nodes $V = \{u \bigcup \mathcal{S}_u^t\}$ and $\mathcal{G}_t^q = \emptyset$
		\FOR{hop $k$ in range $\{1, 2\}$}
		\FORALL{$v$ in $V$}
		\STATE add all neighbors of $v$ in $\mathcal{G}_t$, i.e., $\mathcal{N}_v^t$ to $V$
		\ENDFOR
		\ENDFOR 
		\STATE set the nodes of $\mathcal{G}_t^q$ as $V$
		\FOR{each pair of nodes $(u, v)$ in $\mathcal{G}_t^q$}
		\IF{ $e_{uv} \in \mathcal{G}_t$}
		\STATE add the edge $e_{uv}$ along with its features to $\mathcal{G}_t^q$
		\ENDIF
		\ENDFOR
		\RETURN $\mathcal{G}_t^q$
	\end{algorithmic}
	
	%\vspace{-2em}
\end{algorithm}
As for the edge features,
we first define the item feature $Attr(p)$ as a one-hot vector, where each bin represents a specific range of the price.
Then for an edge $e_{vu}$, its feature $Attr(e_{vu})$ is summed over features of all the items which are sent from the user $v$ to $u$. 
Note that the edge features may change across the queries, since for a specific time span $t$, 
we only sum over item features that are shared between these two users during the period of $t$.
%We use $e_{vu}^t$ to denote the features of the edge $(v,u,)$ in $\mathcal{G}_t^q$. It is the pooling of all \tcode~ sent by user $v$ to user $u$ in time step $t$. We use a simple pooling rule. \hxw{check}We group the Taocode according to their items' similarity with product p. We use four situations to quantify the similarity between product and p: 1)  it is p, 2) it has the same first-category with p, 3) it has the same sep zcond-category with p, 4) others. Then count the total price and total number of each group of product. 
%In our model, the graph's nodes and items have the basic features that are part of our models' input, and we use $ Z $ to denote. The first component in $Z$ is each node's structural label $Z_l$. Our model uses four one-hot labels to mark four kinds of nodes in the dynamic sub-graph:  1) The center node $i$ is the target predict user. 2) The center node $p$ is the target item in prediction. 3) The users $j = \{j_1, j_2,...,j_k\}$ who shared item $p$ are the important nodes in prediction. 4) other nodes. The second component in $Z$ is the users' basic features unrelated to the graph, such as gender, age, height, cost on Taobao.com.  

%The most important is how to preprocessed the diffusion network on the graph. In observation(see 3.3), we can conclude that the direction of the edge is essential. Moreover, know the sender whether purchased the item is also a critical point. So for each Taocodes, we format the features as follows: a) the date receiver purchase, b) the date receiver purchase, c) price of the item. d) category similarity with querys' item  (e.g., whether same in level-1 category). For user $u$ and user $v$, the edge in time step t is the sum of all Taocodes feature that user $u$ share to user $v$ in time step $t$, we use $e_{ij}^t$ to denote.
\subsection{Edge aggregation: \modelname-E}
We then aim to model the \tcode~diffusions given a sequence of diffusion sub-networks with user $u$ as the centered node.
Our general idea is to learn a graph-level representation which contains the information of diffusion patterns of the user;
and traditional GNNs based on message passing~\cite{gin,hgt} first learn the node representations by only aggregating neighborhood features,
since the unattributed edges just represents a specific relationship between pairs of nodes.
However, such kind of methods may not be suitable for our scenario
since the edge features in the \tcode~diffusion network may contain the key properties of a \tcode~sharing,
such as the basic information of the shared products. But if the node only aggregates the features of the edges, it loses some key properties about the graph structure, such as the degree of the node in query. 

Our model first uses a edge-aware GNNs (\modelname-E) with bi-direction graph attention mechanism to aggregate edge features with different weights into the nodes' attributes by time step. We then obtain the graph's global information through a node-aware GNNs (\modelname-N) that aggregates node attributes containing edge information. In this way, our model can capture the local sharing information of the network and the global information of the network. This section will introduce \modelname-E in detail.


%The Graph Neural Networks based on message passing ~\cite{} obtains node attributes by aggregating the information of node neighbors. But this method is not suitable for our situation. Our subnetworks‘ edge features denote the spread of taocodes between the two end nodes of the edge, an essential attribute of these two nodes. Therefore, we first use the aggregation function to merge this edge into the node attributes in chronological order and then perform further representation learning(see 4.2).


 At time step $t$,
 the weight of an edge depends not only on its feature but also on the attributes of two users it connect. 
Simultaneously, the edge features of the two nodes before does also affect the edge weight in time step t. Therefore, our formula is as follows:
\begin{equation}
w^t_{vu} = LeakyReLU(a^T[W^{t-1}e_{vu}^{t-1},W^te_{vu}^{t},h_v^{t-1},h_u^{t-1}])
\end{equation}
Where $W$ denotes the learnable parameters, $a^T$ is a learnable vector.


Next, for easily comparing the coefficients between different nodes, we apply an attention mechanism similar to~\cite{gat}. In our scenario, the softmax operation need \textbf{bi-direction} consideration of two nodes. We use  two softmax functions to get the final weight. One of the softmax functions considers all in-edges of receiving node, and the other considers all out-edges of the sending node:
\begin{equation}
l^t_{vu} = \frac{exp(w_{vu}^t)}{\sum_{k\in \mathcal{S}_u^t} exp(w_{ku}^t)} \label{con:l}
\end{equation}
\begin{equation}
r^t_{vu} = \frac{exp(w_{vu}^t)}{\sum_{k\in \mathcal{R}_{v}^t} exp(w_{vk}^t)}\label{con:r}
\end{equation}
then the two results are multiplied after operating the square:
\begin{equation}
a^t_{vu} = \sqrt{l^t_{vu}}*\sqrt{r^t_{vu}} \label{con:a}
\end{equation}
where $a_{vu}^t$ is the final attention weight of $e_{vu}^t$, 
and the weight obtained by the two-directed considered softmax function can smooth the influence of each node on the surrounding nodes,
similarly as proposed in the \textit{Symmetric Normalized Laplacian}~\cite{chung1997spectral}.

Since the dynamic diffusion sub-network is a directed graph,  
the edge sent from the user is different from the edge received, 
we separately aggregate the node's in- and out- edges:
\begin{equation}
In_u^{t} = \sum_{v\in  \mathcal{S}_u^t} a_{vu}^tW^t e_{vu}^{t}
\end{equation}
\begin{equation}
Out_u^{t} = \sum_{v\in \mathcal{R}_{v}^t} a_{uv}^tW^t e_{uv}^{t}
\end{equation}
where $\mathcal{S}_u$  denotes the set of \textit{sender nodes} that share \tcode~to $u$ in the network, i.e., neighbors of in edges. $\mathcal{R}_u$ is the set of \textit{receiver nodes} that receive \tcode~from $u$ in the network, i.e., neighbors of out edges. 
Then we concatenate them as the final hidden state of user $u$ at the time step $t$.

Taking into account the existence of long-term dependence (see section 3.3), 
we use GRU ~\cite{gru,ggnn} to aggregate the hidden state of each time step of a node:
\begin{equation}
h^{t}_{u} = GRU([In_u^t,Out_u^t], h^{t-1}_u)
\end{equation}
and the initial representation of the node is defined as a linear transformation of the original feature of that node:
	
\begin{equation}
h^{0}_u = ReLU(\Theta^0 * Attr(u))
\end{equation}


Our model supports the multi-head attention mechanism ~\cite{mutihead,gat}. Note that in the calculation of each head, the node attributes are the same. Moreover, for avoiding too many parameters need to be learned, all heads share a same GRU.

After $T$ aggregations, the edge information at all time steps has been aggregated to the node representation. In edge feature aggregation, the attributes of nodes only participate in the calculation of attention weights, and will not directly participate in the aggregation. Therefore, even if there are many time steps, it will not cause excessive smoothness due to mutual aggregation of nodes. 

\subsection{Node aggregation: \modelname-N}
In the edge feature aggregation, since the nodes only participate in the calculation of attention weights and aggregations are not directly applied on nodes, 
we cannot learn the global representation of the graph and nodes' feature of neighbors. 
Therefore, after the edge features at each time step are sequentially aggregated into node features, we need to learn the overall representation of the graph and smooth attributes of nodes through another GNN architecture that can propagate node representations.

Since node attributes could be more important in some scenarios, we add a residual connection~\cite{he2016deep} before the node aggregation:
\begin{equation}
\mathbf{X}^0=\mathbf{H}^{T}+\mathbf{H}^0
\end{equation}

Meanwhile, at this stage, we are more focused on the structure of the network, so we merge the T dynamic interest diffusion networks $\{\mathcal{G}_1^q...\mathcal{G}_T^q\}$ and transformed them into an undirected graph $\mathcal{G}^q$ without edge features. We use $\mathcal{N}_u$ to denote the set of node $u$'s neighbors in $\mathcal{G}^q$.

The formula of a layer in \modelname-N is approximately the same as GAT~\cite{gat}, but when calculating the weight of the edge, we use a two-direction softmax function, see Equation \ref{con:l}, \ref{con:r}, \ref{con:a};
but \modelname-N does not consider the direction of edge, 
the $\mathcal{S}_u^t$ in Equation \ref{con:l}  and the $\mathcal{R}_v^t$ in Equation \ref{con:r} are replaced by $\mathcal{N}_u$ and $\mathcal{N}_v$ respectively. 

After $K$ layers, we can get the final node representation $X^K$. Since there is already an attention mechanism in \modelname-E, we directly average the representations of all nodes in the graph to get the global representation $G_q$ of the network built by query $q$:
\begin{equation}
G_q= \frac{1}{n}\sum_{i=1}^n x_i^{K}
\end{equation}
where $n$ is the number of all node in the network.
\subsection{Downstream tasks}
For predicting user $u$ whether purchase item $p$ in a query $q=(u,p)$, the final representation of the user, the features of the item $p$, and the global representation of the entire network build by query is the vital factors. Moreover, the seed nodes (see section 4.1) are also important for our task, so we average their final representation in Equation \ref{con:e}. 
\begin{equation}
G_q' = \frac{1}{|\mathbf{S}_u(p)|}\sum_{v \in \mathbf{S}_u(p)}x_v^K \label{con:e}
\end{equation}

Then we combine them and output the predictions through a simple linear layer:
\begin{equation}
y' = \mbox{Softmax}(\mbox{Linear}([G_q,G_q',x_u^K, \mbox{Attr}(p)]))
\end{equation}
where $Attr{(p)}$ is the features of item $p$.

In general, our downstream task can be regarded as a problem of binary classification. 
We use the \textit{cross entropy} in our loss function which is defined as follows:
\begin{equation}
\mathcal{L}(\Theta_{all}) = \sum_{q_i \in Q} -y_i \mbox{log}y_i'+(1-y_i)\mbox{log}(1-y_i')
\end{equation}
where $\Theta_{all}$ denotes all learnable parameters in \modelname, $Q$ is the set of all queries, and $y_i$ is the ground truth of the query $q_i$.
